New Physics at the LHC. A Les Houches Report: Physics at TeV Colliders 2009 - New Physics Working Group

We present a collection of signatures for physics beyond the standard model that need to be explored at the LHC. First, are presented various tools developed to measure new particle masses in scenarios where all decays include an unobservable particle. Second, various aspects of supersymmetric models are discussed. Third, some signatures of models of strong electroweak symmetry are discussed. In the fourth part, a special attention is devoted to high mass resonances, as the ones appearing in models with warped extra dimensions. Finally, prospects for models with a hidden sector/valley are presented. Our report, which includes brief experimental and theoretical reviews as well as original results, summarizes the activities of the "New Physics" working group for the "Physics at TeV Colliders" workshop (Les Houches, France, 8-26 June, 2009).

==> Robens/B-L_events.tex <==
Just tree level, generation at detector level still on going.

